A Bayesian method for detecting stellar flares

We present a Bayesian-odds-ratio-based algorithm for detecting stellar flares in light curve data. We assume flares are described by a model in which there is a rapid rise with a half-Gaussian profile, followed by an exponential decay. Our signal model also contains a polynomial background model. This is required to fit underlying light curve variations that are expected in the data, which could otherwise partially mimic a flare. We characterise the false alarm probability and efficiency of this method and compare it with a simpler thresholding method based on that used in Walkowicz et al (2011). We find our method has a significant increase in detection efficiency for low signal-to-noise ratio (S/N) flares. For a conservative false alarm probability our method can detect 95% of flares with S/N less than ~20, as compared to S/N of ~25 for the simpler method. As an example we have applied our method to a selection of stars in Kepler Quarter 1 data. The method finds 687 flaring stars with a total of 1873 flares after vetos have been applied. For these flares we have characterised their durations and and signal-to-noise ratios.

==> restable.tex <==
\hline
\kepler ID & No.\ & $T_{\rm eff}$ & $\log{(g)}$ & Median duration & Median & Median amp. & $\sigma$ \\
~ & flares & (K) & (cm/s$^2$) & (hrs) & \snr & ($e^-/{\rm s}$) & ($e^-/{\rm s}$) \\
\hline
1569863 & 4 & 3809 & 4.45 & 3.14 & 11.01 & 55.79 & 5.9 \\
1570924 & 3 & 4923 & 4.55 & 2.99 & 64.85 & 3774.86 & 59.5 \\
1722506 & 2 & 4270 & 4.43 & 12.20 & 68.62 & 963.49 & 9.8 \\
1873543 & 2 & 3702 & 4.52 & 4.33 & 25.76 & 176.47 & 8.0 \\
2013754 & 5 & 4280 & 4.57 & 4.55 & 12.06 & 79.42 & 7.8 \\
2140782 & 1 & 4946 & 4.62 & 2.35 & 12.87 & 77.39 & 5.1 \\
2437317 & 1 & 4250 & 4.70 & 7.49 & 575.65 & 2574.92 & 8.6 \\
2441562 & 1 & 3806 & 4.46 & 4.49 & 37.02 & 149.61 & 5.0 \\
2442866 & 3 & 4344 & 4.49 & 9.44 & 14.56 & 62.76 & 8.6 \\
2570846 & 1 & 3865 & 4.61 & 2.62 & 24.98 & 152.08 & 5.3 \\
\hline

